Learning Regional Attraction for Line Segment Detection

This paper presents regional attraction of line segment maps, and hereby poses the problem of line segment detection (LSD) as a problem of region coloring. Given a line segment map, the proposed regional attraction first establishes the relationship between line segments and regions in the image lattice. Based on this, the line segment map is equivalently transformed to an attraction field map (AFM), which can be remapped to a set of line segments without loss of information. Accordingly, we develop an end-to-end framework to learn attraction field maps for raw input images, followed by a squeeze module to detect line segments. Apart from existing works, the proposed detector properly handles the local ambiguity and does not rely on the accurate identification of edge pixels. Comprehensive experiments on the Wireframe dataset and the YorkUrban dataset demonstrate the superiority of our method. In particular, we achieve an F-measure of 0.831 on the Wireframe dataset, advancing the state-of-the-art performance by 10.3 percent.

==> 2_Regional Attraction Final_PAMI/figures/offset_details.tex <==
\begin{tikzpicture}[scale=0.33]
\pgfmathsetmacro{\ymin}{0}
\pgfmathsetmacro{\xmin}{0}
\pgfmathsetmacro{\ymax}{6}
\pgfmathsetmacro{\xmax}{7}	
\foreach \i in {\xmin,...,\xmax} {
		\draw [thick, gray] (\i, \ymin) -- (\i, \ymax) node [below] at (\i, \ymin) {};
	}
\foreach \i in {\ymin,\ymax} {
	\draw [thick, gray] (\xmin, \i) -- (\xmax, \i) node [below] at (\xmin, \i) {};
    }
% 	\foreach \x in {\xmin,...,\xmax-1}
%             \foreach \y in {\ymin,...,\ymax-1}
%                 \node [circle, fill, inner sep=0.5pt, gray]  (\x\y) at (\x+0.5,\y+0.5) {}; 
\draw [step=1.0, black] (\xmin, \ymin) grid (\xmax,\ymax);
\node[circle, fill, inner sep=1.0pt, blue] (A) at (1.73,4.29) {};
\node[circle, fill, inner sep=1.0pt, blue] (B) at (5.60,1.40) {};
\draw [red, very thick] (A) -- (B);
\fill [green, opacity=0.2] (0,0) -- (7,0) -- (7,3) -- (6,3) -- (6,5) -- (4,5) -- (4,6) -- (0,6) -- (0,0);

\node[circle, fill, inner sep=0.5pt, gray](ea1) at (0.5,5.5) {};
\node[circle, fill, inner sep=0.5pt, gray](ea2) at (1.5,5.5) {};
\node[circle, fill, inner sep=0.5pt, gray](ea3) at (0.5,4.5) {};
\node[circle, fill, inner sep=0.5pt, gray](ea4) at (1.5,4.5) {};
\node[circle, fill, inner sep=0.5pt, gray](ea5) at (0.5,3.5) {};
\node[circle, fill, inner sep=0.5pt, blue](ea6) at (2.5,5.5) {};
\node[circle, fill, inner sep=0.5pt, gray](eb1) at (6.5,2.5) {};
\node[circle, fill, inner sep=0.5pt, gray](eb2) at (6.5,1.5) {};
\node[circle, fill, inner sep=0.5pt, gray](eb3) at (6.5,0.5) {};
\node[circle, fill, inner sep=0.5pt, gray](eb4) at (5.5,0.5) {};
\node[circle, fill, inner sep=0.5pt, blue](c3) at (1.5,1.5) {};
\node[circle, fill, inner sep=0.5pt, blue](d2) at (2.5,1.5) {};
\node[circle, fill, inner sep=0.5pt, blue](e4) at (3.5,3.5) {};
\node[circle, fill, inner sep=0.5pt, blue](f1) at (4.5,0.5) {};
\node[circle, fill, inner sep=0.5pt, blue](f2) at (4.5,1.5) {};	
\node[circle, fill, inner sep=0.5pt, blue](g3) at (5.5,4.5)  {};	
\draw [->,>=stealth, dashed, thick] (ea1) -- (A);
\draw [->,>=stealth, dashed, thick] (ea2) -- (A);
\draw [->,>=stealth, dashed, thick] (ea3) -- (A);
\draw [->,>=stealth, dashed, thick] (ea4) -- (A);
\draw [->,>=stealth, dashed, thick] (ea5) -- (A);
\draw [->,>=stealth, dashed, thick] (ea6) -- (A);
\draw [->,>=stealth, dashed, thick] (eb1) -- (B);
\draw [->,>=stealth, dashed, thick] (eb2) -- (B);
\draw [->,>=stealth, dashed, thick] (eb3) -- (B);
\draw [->,>=stealth, dashed, thick] (eb4) -- (B);
\draw [->,>=stealth, thick] (c3) -- ($(A)!(c3)!(B)$);
\draw [->,>=stealth, thick] (d2) -- ($(A)!(d2)!(B)$);
\draw [->,>=stealth, thick] (e4) -- ($(A)!(e4)!(B)$);
\draw [->,>=stealth, thick] (f1) -- ($(A)!(f1)!(B)$);
\draw [->,>=stealth, thick] (f2) -- ($(A)!(f2)!(B)$);
\draw [->,>=stealth, thick] (g3) -- ($(A)!(g3)!(B)$);
\end{tikzpicture}

==> 2_Regional Attraction Final_PAMI/figures/squeeze.tex <==
\begin{tikzpicture}[scale=0.33]
\pgfmathsetmacro{\ymin}{0}
\pgfmathsetmacro{\xmin}{0}
\pgfmathsetmacro{\ymax}{6}
\pgfmathsetmacro{\xmax}{7}	
\foreach \i in {\xmin,...,\xmax} {
		\draw [thick, gray, opacity=0] (\i, \ymin) -- (\i, \ymax) node [below] at (\i, \ymin) {};
	}
\foreach \i in {\ymin,\ymax} {
	\draw [thick, gray] (\xmin, \i) -- (\xmax, \i) node [below] at (\xmin, \i) {};
    }
% 	\foreach \x in {\xmin,...,\xmax-1}
%             \foreach \y in {\ymin,...,\ymax-1}
%                 \node [circle, fill, inner sep=0.5pt, gray]  (\x\y) at (\x+0.5,\y+0.5) {}; 
\draw [step=1.0, black] (\xmin, \ymin) grid (\xmax,\ymax);
\node[inner sep=1.0pt, blue] (A) at (1.73,4.29) {};
\node[inner sep=1.0pt, blue] (B) at (5.60,1.40) {};
% \draw [red, very thick] (A) -- (B);
% \fill [green, opacity=0.2] (0,0) -- (7,0) -- (7,3) -- (6,3) -- (6,5) -- (4,5) -- (4,6) -- (0,6) -- (0,0);
% \draw (A) -- (B);
\coordinate (dir) at (-0.26708016,  0.19944745);
\node[inner sep=0.5pt] (a0) at (0.5, 0.5) {};
\node[inner sep=0.5pt] (a0p) at ($(A)!(a0)!(B)$){};
\draw[->] (a0p) -- ++(dir);
\node[inner sep=0.5pt] (a1) at (1.5, 0.5){};
\node[inner sep=0.5pt] (a1p) at ($(A)!(a1)!(B)$){};
\draw[->] (a1p) -- ++(dir);
\node[inner sep=0.5pt] (a2) at (2.5, 0.5){};
\node[inner sep=0.5pt] (a2p) at ($(A)!(a2)!(B)$){};
\draw[->] (a2p) -- ++(dir);
\node[inner sep=0.5pt] (a3) at (3.5, 0.5){};
\node[inner sep=0.5pt] (a3p) at ($(A)!(a3)!(B)$){};
\draw[->] (a3p) -- ++(dir);
\node[inner sep=0.5pt] (a4) at (4.5, 0.5){};
\node[inner sep=0.5pt] (a4p) at ($(A)!(a4)!(B)$){};
\draw[->] (a4p) -- ++(dir);
\node[inner sep=0.5pt] (a5) at (0.5, 1.5){};
\node[inner sep=0.5pt] (a5p) at ($(A)!(a5)!(B)$){};
\draw[->] (a5p) -- ++(dir);
\node[inner sep=0.5pt] (a6) at (1.5, 1.5){};
\node[inner sep=0.5pt] (a6p) at ($(A)!(a6)!(B)$){};
\draw[->] (a6p) -- ++(dir);
\node[inner sep=0.5pt] (a7) at (2.5, 1.5){};
\node[inner sep=0.5pt] (a7p) at ($(A)!(a7)!(B)$){};
\draw[->] (a7p) -- ++(dir);
\node[inner sep=0.5pt] (a8) at (3.5, 1.5){};
\node[inner sep=0.5pt] (a8p) at ($(A)!(a8)!(B)$){};
\draw[->] (a8p) -- ++(dir);
\node[inner sep=0.5pt] (a9) at (4.5, 1.5){};
\node[inner sep=0.5pt] (a9p) at ($(A)!(a9)!(B)$){};
\draw[->] (a9p) -- ++(dir);
\node[inner sep=0.5pt] (a10) at (0.5, 2.5){};
\node[inner sep=0.5pt] (a10p) at ($(A)!(a10)!(B)$){};
\draw[->] (a10p) -- ++(dir);
\node[inner sep=0.5pt] (a11) at (1.5, 2.5){};
\node[inner sep=0.5pt] (a11p) at ($(A)!(a11)!(B)$){};
\draw[->] (a11p) -- ++(dir);
\node[inner sep=0.5pt] (a12) at (2.5, 2.5){};
\node[inner sep=0.5pt] (a12p) at ($(A)!(a12)!(B)$){};
\draw[->] (a12p) -- ++(dir);
\node[inner sep=0.5pt] (a13) at (3.5, 2.5){};
\node[inner sep=0.5pt] (a13p) at ($(A)!(a13)!(B)$){};
\draw[->] (a13p) -- ++(dir);
\node[inner sep=0.5pt] (a14) at (4.5, 2.5){};
\node[inner sep=0.5pt] (a14p) at ($(A)!(a14)!(B)$){};
\draw[->] (a14p) -- ++(dir);
\node[inner sep=0.5pt] (a15) at (5.5, 2.5){};
\node[inner sep=0.5pt] (a15p) at ($(A)!(a15)!(B)$){};
\draw[->] (a15p) -- ++(dir);
\node[inner sep=0.5pt] (a16) at (1.5, 3.5){};
\node[inner sep=0.5pt] (a16p) at ($(A)!(a16)!(B)$){};
\draw[->] (a16p) -- ++(dir);
\node[inner sep=0.5pt] (a17) at (2.5, 3.5){};
\node[inner sep=0.5pt] (a17p) at ($(A)!(a17)!(B)$){};
\draw[->] (a17p) -- ++(dir);
\node[inner sep=0.5pt] (a18) at (3.5, 3.5){};
\node[inner sep=0.5pt] (a18p) at ($(A)!(a18)!(B)$){};
\draw[->] (a18p) -- ++(dir);
\node[inner sep=0.5pt] (a19) at (4.5, 3.5){};
\node[inner sep=0.5pt] (a19p) at ($(A)!(a19)!(B)$){};
\draw[->] (a19p) -- ++(dir);
\node[inner sep=0.5pt] (a20) at (5.5, 3.5){};
\node[inner sep=0.5pt] (a20p) at ($(A)!(a20)!(B)$){};
\draw[->] (a20p) -- ++(dir);
\node[inner sep=0.5pt] (a21) at (1.5, 4.5){};
\node[inner sep=0.5pt] (a21p) at ($(A)!(a21)!(B)$){};
\draw[->] (a21p) -- ++(dir);
\node[inner sep=0.5pt] (a22) at (2.5, 4.5){};
\node[inner sep=0.5pt] (a22p) at ($(A)!(a22)!(B)$){};
\draw[->] (a22p) -- ++(dir);
\node[inner sep=0.5pt] (a23) at (3.5, 4.5){};
\node[inner sep=0.5pt] (a23p) at ($(A)!(a23)!(B)$){};
\draw[->] (a23p) -- ++(dir);
\node[inner sep=0.5pt] (a24) at (4.5, 4.5){};
\node[inner sep=0.5pt] (a24p) at ($(A)!(a24)!(B)$){};
\draw[->] (a24p) -- ++(dir);
\node[inner sep=0.5pt] (a25) at (5.5, 4.5){};
\node[inner sep=0.5pt] (a25p) at ($(A)!(a25)!(B)$){};
\draw[->] (a25p) -- ++(dir);
\draw [red,opacity=0.5,->] (A) -- ++(-0.35643939549437625, 0.3506436329660124);
\draw [red,opacity=0.5,->] (A) -- ++(-0.09336950361691489, 0.4912047798976827);
\draw [red,opacity=0.5,->] (A) -- ++(-0.4928682127552036, 0.08414823144601036);
\draw [red,opacity=0.5,->] (A) -- ++(-0.36924274696406295, 0.33713468201066615);
\draw [red,opacity=0.5,->] (A) -- ++(-0.42070033194990575, -0.2702059042605086);
\draw [red,opacity=0.5,->] (A) -- ++(0.26843774609657967, 0.42183074386605374);
\draw [red,opacity=0.5,->] (5.6, 1.4) -- ++(-0.3166188951286314, -0.38697864960166045);
\draw [red,opacity=0.5,->] (5.6, 1.4) -- ++(-0.4969418673368095, -0.0552157630374233);
\draw [red,opacity=0.5,->] (5.6, 1.4) -- ++(-0.35355339059327384, 0.3535533905932737);
\draw [red,opacity=0.5,->] (5.6, 1.4) -- ++(0.055215763037423087, 0.4969418673368095);
\fill[green,opacity=0.2] (1.0, 4.0) rectangle (2.0, 5.0);
\fill[green,opacity=0.2] (2.0, 4.0) rectangle (3.0, 5.0);
\fill[green,opacity=0.2] (2.0, 3.0) rectangle (3.0, 4.0);
\fill[green,opacity=0.2] (3.0, 3.0) rectangle (4.0, 4.0);
\fill[green,opacity=0.2] (3.0, 2.0) rectangle (4.0, 3.0);
\fill[green,opacity=0.2] (4.0, 2.0) rectangle (5.0, 3.0);
\fill[green,opacity=0.2] (4.0, 1.0) rectangle (5.0, 2.0);
\fill[green,opacity=0.2] (5.0, 1.0) rectangle (6.0, 2.0);
\end{tikzpicture}

==> 2_Regional Attraction Final_PAMI/figures/support_region.tex <==
\begin{tikzpicture}[scale=0.2]
        % \node[anchor=south west,inner sep=0] at (0,0)
        % {\includegraphics[width=1.2\linewidth]{figures/occup.png}};
        \pgfmathsetmacro{\ymin}{0}
        \pgfmathsetmacro{\xmin}{0}
        \pgfmathsetmacro{\ymax}{10}
        \pgfmathsetmacro{\xmax}{10}	
        \node[circle, fill, inner sep=1.0pt, red] (A0) at (2.36,8.1) {};
        \node[circle, fill, inner sep=1.0pt, red] (A1) at (7.23,6.83) {};
        \node[circle, fill, inner sep=1.0pt, green] (B0) at (8,1.2) {};
        \node[circle, fill, inner sep=1.0pt, green] (B1) at (8.7,6.5) {};
        \node[circle, fill, inner sep=1.0pt, blue] (C0) at (1.73,4.29) {};
        \node[circle, fill, inner sep=1.0pt, blue] (C1) at (5.60,1.40) {};
        
        \draw [blue, very thick] (A0) -- (A1);	
        \draw [green, very thick] (B0) -- (B1);
        \draw [red, very thick] (C0) -- (C1);

        \foreach \i in {\xmin,\xmax} {
			\draw [thick, gray] (\i, \ymin) -- (\i, \ymax) node [below] at (\i, \ymin) {};
		}
		\foreach \i in {\ymin,\ymax} {
		\draw [thick, gray] (\xmin, \i) -- (\xmax, \i) node [below] at (\xmin, \i) {};
	    }        
        \draw [step=1.0, black] (\xmin, \ymin) grid (\xmax,\ymax);

        % \foreach \x in {\xmin,...,\xmax-1}
        %     \foreach \y in {\ymin,...,\ymax-1}
        %         \node [circle, fill, inner sep=0.5pt, gray]  (\x\y) at (\x+0.5,\y+0.5) {}; 
        \fill [green, opacity=0.2] (0,0) -- (7,0) -- (7,3) -- (6,3) -- (6,5) -- (4,5) -- (4,6) -- (0,6) -- (0,0);
        \fill [red, opacity=0.2] (6,5) -- (6,3) -- (7,3) -- (7,0) -- (10,0) -- (10,10) -- (9,10) -- (9,9) -- (8,9) -- (8,8) -- (8,7) -- (8,6) -- (7,6) -- (7,5) -- (6,5);
        \fill [blue, opacity=0.2] (0,6) -- (4,6) -- (4,5) -- (7,5) -- (7,6) -- (8,6) -- (8,9) -- (9,9) -- (9,10) -- (0,10) -- (0,6);
        \end{tikzpicture}

==> 2_Regional Attraction Final_PAMI/ieeebst <==

% ---------------------------------------------------------------
%
% ieee.bst,v 1.0 2002/04/16
%
% by Glenn Paulley (paulley@acm.org)
%
% Modified from latex8.bst 1995/09/15 15:13:49 ienne Exp $
%
% by Paolo.Ienne@di.epfl.ch
%
%
% ---------------------------------------------------------------
%
% no guarantee is given that the format corresponds perfectly to 
% IEEE 8.5" x 11" Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------
%
% `ieee' from BibTeX standard bibliography style `abbrv'
% version 0.99a for BibTeX versions 0.99a or later, LaTeX version 2.09.
% Copyright (C) 1985, all rights reserved.
% Copying of this file is authorized only if either
% (1) you make absolutely no changes to your copy, including name, or
% (2) if you do make changes, you name it something other than
% btxbst.doc, plain.bst, unsrt.bst, alpha.bst, and abbrv.bst.
% This restriction helps ensure that all standard styles are identical.
% The file btxbst.doc has the documentation for this style.

ENTRY
  { address
    author
    booktitle
    chapter
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
  }
  {}
  { label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
 { add.period$ write$
   newline$
   "\newblock " write$
 }
 { output.state before.all =
     'write$
     { add.period$ " " * write$ }
   if$
 }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem{" write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
 'skip$
 { after.sentence 'output.state := }
      if$
    }
  if$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {new.block.checka}
{ empty$
    'skip$
    'new.block
  if$
}

FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}

FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}

FUNCTION {new.sentence.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.sentence
  if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "{\em " swap$ * "}" * }
  if$
}

INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 's :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr "{f.~}{vv~}{ll}{, jj}" format.name$ 't :=
      nameptr #1 >
 { namesleft #1 >
     { ", " * t * }
     { numnames #2 >
  { "," * }
  'skip$
       if$
       t "others" =
  { " et~al." * }
  { " and " * t * }
       if$
     }
   if$
 }
 't
      if$
      nameptr #1 + 'nameptr :=

      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
    { "" }
    { editor format.names
      editor num.names$ #1 >
 { ", editors" * }
 { ", editor" * }
      if$
    }
  if$
}

FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}

FUNCTION {n.dashify}
{ 't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
 { t #1 #2 substring$ "--" = not
     { "--" *
       t #2 global.max$ substring$ 't :=
     }
     {   { t #1 #1 substring$ "-" = }
  { "-" *
    t #2 global.max$ substring$ 't :=
  }
       while$
     }
   if$
 }
 { t #1 #1 substring$ *
   t #2 global.max$ substring$ 't :=
 }
      if$
    }
  while$
}

FUNCTION {format.date}
{ year empty$
    { month empty$
 { "" }
 { "there's a month but no year in " cite$ * warning$
   month
 }
      if$
    }
    { month empty$
 'year
 { month " " * year * }
      if$
    }
  if$
}

FUNCTION {format.btitle}
{ title emphasize
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}

FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { "volume" volume tie.or.space.connect
      series empty$
 'skip$
 { " of " * series emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION {format.number.series}
{ volume empty$
    { number empty$
 { series field.or.null }
 { output.state mid.sentence =
     { "number" }
     { "Number" }
   if$
   number tie.or.space.connect
   series empty$
     { "there's a number but no series in " cite$ * warning$ }
     { " in " * series * }
   if$
 }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { output.state mid.sentence =
 { edition "l" change.case$ " edition" * }
 { edition "t" change.case$ " edition" * }
      if$
    }
  if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
 { #1 'multiresult := }
 { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { pages multi.page.check
 { "pages" pages n.dashify tie.or.space.connect }
 { "page" pages tie.or.space.connect }
      if$
    }
  if$
}

FUNCTION {format.vol.num.pages}
{ volume field.or.null
  number empty$
    'skip$
    { "(" number * ")" * *
      volume empty$
 { "there's a number but no volume in " cite$ * warning$ }
 'skip$
      if$
    }
  if$
  pages empty$
    'skip$
    { duplicate$ empty$
 { pop$ format.pages }
 { ":" * pages n.dashify * }
      if$
    }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
 { "chapter" }
 { type "l" change.case$ }
      if$
      chapter tie.or.space.connect
      pages empty$
 'skip$
 { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
    { "" }
    { editor empty$
 { "In " booktitle emphasize * }
 { "In " format.editors * ", " * booktitle emphasize * }
      if$
    }
  if$
}

FUNCTION {empty.misc.check}

{ author empty$ title empty$ howpublished empty$
  month empty$ year empty$ note empty$
  and and and and and
  key empty$ not and
    { "all relevant fields are empty in " cite$ * warning$ }
    'skip$
  if$
}

FUNCTION {format.thesis.type}
{ type empty$
    'skip$
    { pop$
      type "t" change.case$
    }
  if$
}

FUNCTION {format.tr.number}
{ type empty$
    { "Technical Report" }
    'type
  if$
  number empty$
    { "t" change.case$ }
    { number tie.or.space.connect }
  if$
}

FUNCTION {format.article.crossref}
{ key empty$
    { journal empty$
 { "need key or journal for " cite$ * " to crossref " * crossref *
   warning$
   ""
 }
 { "In {\em " journal * "\/}" * }
      if$
    }
    { "In " key * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
  editor num.names$ duplicate$
  #2 >
    { pop$ " et~al." * }
    { #2 <
 'skip$
 { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
     { " et~al." * }
     { " and " * editor #2 "{vv~}{ll}" format.name$ * }
   if$
 }
      if$
    }
  if$
}

FUNCTION {format.book.crossref}
{ volume empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      "In "
    }
    { "Volume" volume tie.or.space.connect
      " of " *
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { series empty$
     { "need editor, key, or series for " cite$ * " to crossref " *
       crossref * warning$
       "" *
     }
     { "{\em " * series * "\/}" * }
   if$
 }
 { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { booktitle empty$
     { "need editor, key, or booktitle for " cite$ * " to crossref " *
       crossref * warning$
       ""
     }
     { "In {\em " booktitle * "\/}" * }
   if$
 }
 { "In " key * }
      if$
    }
    { "In " format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { journal emphasize "journal" output.check
      format.vol.num.pages output
      format.date "year" output.check
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull
      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  format.authors output
  new.block
  format.title "title" output.check
  howpublished address new.block.checkb
  howpublished output
  address output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull

      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.chapter.pages output
      new.sentence
      publisher "publisher" output.check
      address output
      format.edition output
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.pages output
      address empty$
 { organization publisher new.sentence.checkb
   organization output
   publisher output
   format.date "year" output.check
 }
 { address output.nonnull
   format.date "year" output.check
   new.sentence
   organization output
   publisher output
 }
      if$
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization empty$
 'skip$
 { organization output.nonnull
   address output
 }
      if$
    }
    { format.authors output.nonnull }
  if$
  new.block
  format.btitle "title" output.check
  author empty$
    { organization empty$
 { address new.block.checka
   address output
 }
 'skip$
      if$
    }
    { organization address new.block.checkb
      organization output
      address output
    }
  if$
  format.edition output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  "Master's thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  title howpublished new.block.checkb
  format.title output
  howpublished new.block.checka
  howpublished output
  format.date output
  new.block
  note output
  fin.entry
  empty.misc.check
}

FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.btitle "title" output.check
  new.block
  "PhD thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization output }
    { format.editors output.nonnull }

  if$
  new.block
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  address empty$
    { editor empty$
 { publisher new.sentence.checka }
 { organization publisher new.sentence.checkb
   organization output
 }
      if$
      publisher output
      format.date "year" output.check
    }
    { address output.nonnull
      format.date "year" output.check
      new.sentence
      editor empty$
 'skip$
 { organization output }
      if$
      publisher output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  note "note" output.check
  format.date output
  fin.entry
}

FUNCTION {default.type} { misc }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sept."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Softw. Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput.-Aided Design Integrated Circuits"}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Programming"}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Gr."}

MACRO {toms} {"ACM Trans. Math. Softw."}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Prog. Lang. Syst."}

MACRO {tcs} {"Theoretical Comput. Sci."}

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
 { "   " * }
 'skip$
      if$
      s nameptr "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
 { "et al" * }
 { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
 { "to sort, need author or key in " cite$ * warning$
   ""
 }
 { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
 { key empty$
     { "to sort, need author, editor, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.organization.sort}
{ author empty$

    { organization empty$
 { key empty$
     { "to sort, need author, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.organization.sort}
{ editor empty$
    { organization empty$
 { key empty$
     { "to sort, need editor, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {presort}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
 'editor.organization.sort
 { type$ "manual" =
     'author.organization.sort
     'author.sort
   if$
 }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { longest.label }

INTEGERS { number.label longest.label.width }

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #1 'number.label :=
  #0 'longest.label.width :=
}

FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
  number.label #1 + 'number.label :=
  label width$ longest.label.width >
    { label 'longest.label :=
      label width$ 'longest.label.width :=
    }
    'skip$
  if$
}

EXECUTE {initialize.longest.label}

ITERATE {longest.label.pass}

FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{"  longest.label  * "}" *
  "\itemsep=-1pt" * % Compact the entries a little.
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}

% end of file ieee.bst
% ---------------------------------------------------------------





==> 2_Regional Attraction Final_PAMI/teaser.tex <==
\begin{figure}
    \centering
    \subfigure[Input\label{fig:teaser-input}]{
    \includegraphics[width=0.35\linewidth]{figures/teaser/image.png}}
    \subfigure[Ours\label{fig:teaser-ours}]{
    \includegraphics[width=0.59\linewidth]{figures/teaser/our}
    }\\
% \vspace{-3mm}
    \subfigure[Local Edge Map\label{fig:teaser-local-edge}]{
    \includegraphics[width=0.35\linewidth]{figures/teaser/local_edgemap.png}}
    \subfigure[MCMLSD~\cite{Almazan_2017_CVPR}\label{fig:teaser-mcmlsd}]{
    \includegraphics[width=0.59\linewidth]{figures/teaser/mcmlsd}}\\
% \vspace{-3mm}
    \subfigure[Gradient Magnitude\label{fig:teaser-gradient}]{
    \includegraphics[width=0.35\linewidth]{figures/teaser/gradient_mag.png}}
    \subfigure[LSD~\cite{VonGioi2010}\label{fig:teaser-lsd}]{\includegraphics[width=0.59\linewidth]{figures/teaser/lsd}}\\
% \vspace{-3mm}
    \subfigure[Deep Edge Map\label{fig:teaser-deep-edge}]{
    \includegraphics[width=0.35\linewidth]{figures/teaser/deep_edgemap.png}
    }
    \subfigure[DWP~\cite{Huang2018a}\label{fig:teaser-dwp}]{\includegraphics[width=0.59\linewidth]{figures/teaser/wireframe}}
\vspace{-2mm}    
    \caption{Illustrative examples of different methods on an image (a). (b) shows our detected line segments. (c) and (d) present the locally estimated edge map and the result of MCMLSD~\cite{Almazan_2017_CVPR}. (e) and (f) present the gradient magnitude and the result of LSD~\cite{VonGioi2010}. (g) and (h) display the deep edge map and the result of Deep Wireframe Parser (DWP)~\cite{Huang2018a}. The rightmost column shows the close-up (in red) of detection results by different methods, which highlights the better accuracy of our proposed method. Best viewed in color.}
    \label{fig:my_label}
\end{figure}

%      of the proposed line segment detector. In the first row: (a) shows an example test image in the Wireframe dataset~\cite{Huang2018a}; (b) displays the detected line segments by our method;     As a comparison, the last three rows display the used edge cues and corresponding detection results by different approaches. In detail, the locally estimated edge map shown in (c) is used by MCMLSD~\cite{Almazan_2017_CVPR} to obtain the result in (d); The gradient magnitude and the result of LSD~\cite{VonGioi2010} are displayed in (e) and (f) respectively;  Deep Wireframe Parser (DWP)~\cite{Huang2018a} takes the deep edge map (shown in (g)) to get the result of (h).

==> 2_Regional Attraction Final_PAMI/wireframe_vis.tex <==
\begin{figure*}[ht!]
\centering
\def\outsize{0.13\textheight}
\def\xshift{-4mm}
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {LSD};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_lsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_lsd}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_lsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_lsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_lsd}
\\
% }
% \subfigure[MCMLSD \cite{Almazan_2017_CVPR}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {MCMLSD};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_mcmlsd}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_mcmlsd}
\\
% }
% \subfigure[Linelet \cite{Cho2018}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {Linelet};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_linelet}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_linelet}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_linelet}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_linelet}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_linelet}

% \subfigure[Wireframe Parser \cite{Huang2018a}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {DWP};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_wireframe}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_wireframe}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_wireframe}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_wireframe}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_wireframe}

% }
% \subfigure[Ours (a-trous Residual U-Net)]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {AFM};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_ours}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_ours}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_ours}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_ours}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_ours}
% }

\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {AFM++};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577}
% }

% \begin{rotate}{90}
% % \hspace{-20pt}
% GT
% \end{rotate}
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (GT) at (0,0) {GT};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
\includegraphics[height=\outsize]{\resultspath/wireframe/00070841_gt}
\includegraphics[height=\outsize]{\resultspath/wireframe/00190181_gt}
%\includegraphics[height=\outsize]{figures/results/wireframe/00192219_gt}
\includegraphics[height=\outsize]{\resultspath/wireframe/00247823_gt}
\includegraphics[height=\outsize]{\resultspath/wireframe/00491577_gt}
\caption{Some results of line segment detection of different approaches on the Wireframe \cite{Huang2018a} dataset. From top to bottom: LSD \cite{VonGioi2010}, MCMLSD \cite{Almazan_2017_CVPR}, Linelet \cite{Cho2018}, DWP~\cite{Huang2018a}, AFM~\cite{AFMCVPR} with the \emph{a-trous} Residual U-Net and AFM++ proposed in this paper. %Threshold configuration for visualization: (1) The \emph{a-contrario} validation of LSD and Linelet are set as $-\log\epsilon = 0.01\cdot1.75^{8}$; (2) The top $90$ detected line segments for the MCMLSD are visualized; (3) The threshold for line heat map is $10$ for the deep wireframe parser; (4) The upper bound of aspect ratio is set as $0.2$ for our results.
}
\label{fig:results_wireframe}
\vspace{-3mm}
\end{figure*}

==> 2_Regional Attraction Final_PAMI/yorkurban_vis.tex <==
\begin{figure*}[ht!]
\centering
\def\outsize{0.13\textheight}
\def\xshift{-4mm}
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {LSD};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_lsd}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_lsd}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_lsd}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_lsd}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_lsd}
\\
% }
% \subfigure[MCMLSD \cite{Almazan_2017_CVPR}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {MCMLSD};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_mcmlsd}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_mcmlsd}
\\
% }
% \subfigure[Linelet \cite{Cho2018}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {Linelet};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_linelet}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_linelet}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_linelet}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_linelet}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_linelet}


% \subfigure[Wireframe Parser \cite{Huang2018a}]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {DWP};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_wireframe}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_wireframe}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_wireframe}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_wireframe}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_wireframe}

% }
% \subfigure[Ours (a-trous Residual U-Net)]{
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {AFM};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_ours}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_ours}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_ours}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_ours}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_ours}
% }

\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (Ours) at (0,0) {AFM++};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826}
\includegraphics[height=\outsize]{\resultspath/york/P1020847}
\includegraphics[height=\outsize]{\resultspath/york/P1040817}
\includegraphics[height=\outsize]{\resultspath/york/P1040829}
\includegraphics[height=\outsize]{\resultspath/york/P1080084}
% }

% \begin{rotate}{90}
% % \hspace{-20pt}
% GT
% \end{rotate}
\hspace{\xshift}
\begin{tikzpicture}
\node[rotate=90] (GT) at (0,0) {GT};
\draw[opacity=0] (-\outsize*0.01,-\outsize*0.5) rectangle (\outsize*0.01,\outsize*0.5);
\end{tikzpicture}
%\includegraphics[height=\outsize]{figures/results/york/P1020826_gt}
\includegraphics[height=\outsize]{\resultspath/york/P1020847_gt}
\includegraphics[height=\outsize]{\resultspath/york/P1040817_gt}
\includegraphics[height=\outsize]{\resultspath/york/P1040829_gt}
\includegraphics[height=\outsize]{\resultspath/york/P1080084_gt}

\caption{Some results of line segment detection of different approaches on the YorkUrban \cite{Denis2008} datasets. From top to bottom: LSD \cite{VonGioi2010}, MCMLSD \cite{Almazan_2017_CVPR}, Linelet \cite{Cho2018}, DWP \cite{Huang2018a}, AFM~\cite{AFMCVPR} with the \emph{a-trous} Residual U-Net and AFM++ proposed in this paper. 
%Threshold configuration for visualization: (1) The \emph{a-contrario} validation of LSD and Linelet are set as $-\log\epsilon = 0.01\cdot1.75^{8}$; (2) The top $90$ detected line segments for the MCMLSD are visualized; (3) The threshold for line heat map is $10$ for the deep wireframe parser; (4) The upper bound of aspect ratio is set as $0.2$ for our results.
}
\label{fig:results_york}
\vspace{-3mm}
\end{figure*}

==> ieeebst <==

% ---------------------------------------------------------------
%
% ieee.bst,v 1.0 2002/04/16
%
% by Glenn Paulley (paulley@acm.org)
%
% Modified from latex8.bst 1995/09/15 15:13:49 ienne Exp $
%
% by Paolo.Ienne@di.epfl.ch
%
%
% ---------------------------------------------------------------
%
% no guarantee is given that the format corresponds perfectly to 
% IEEE 8.5" x 11" Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------
%
% `ieee' from BibTeX standard bibliography style `abbrv'
% version 0.99a for BibTeX versions 0.99a or later, LaTeX version 2.09.
% Copyright (C) 1985, all rights reserved.
% Copying of this file is authorized only if either
% (1) you make absolutely no changes to your copy, including name, or
% (2) if you do make changes, you name it something other than
% btxbst.doc, plain.bst, unsrt.bst, alpha.bst, and abbrv.bst.
% This restriction helps ensure that all standard styles are identical.
% The file btxbst.doc has the documentation for this style.

ENTRY
  { address
    author
    booktitle
    chapter
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
  }
  {}
  { label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
 { add.period$ write$
   newline$
   "\newblock " write$
 }
 { output.state before.all =
     'write$
     { add.period$ " " * write$ }
   if$
 }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem{" write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
 'skip$
 { after.sentence 'output.state := }
      if$
    }
  if$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {new.block.checka}
{ empty$
    'skip$
    'new.block
  if$
}

FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}

FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}

FUNCTION {new.sentence.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.sentence
  if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "{\em " swap$ * "}" * }
  if$
}

INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 's :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr "{f.~}{vv~}{ll}{, jj}" format.name$ 't :=
      nameptr #1 >
 { namesleft #1 >
     { ", " * t * }
     { numnames #2 >
  { "," * }
  'skip$
       if$
       t "others" =
  { " et~al." * }
  { " and " * t * }
       if$
     }
   if$
 }
 't
      if$
      nameptr #1 + 'nameptr :=

      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
    { "" }
    { editor format.names
      editor num.names$ #1 >
 { ", editors" * }
 { ", editor" * }
      if$
    }
  if$
}

FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}

FUNCTION {n.dashify}
{ 't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
 { t #1 #2 substring$ "--" = not
     { "--" *
       t #2 global.max$ substring$ 't :=
     }
     {   { t #1 #1 substring$ "-" = }
  { "-" *
    t #2 global.max$ substring$ 't :=
  }
       while$
     }
   if$
 }
 { t #1 #1 substring$ *
   t #2 global.max$ substring$ 't :=
 }
      if$
    }
  while$
}

FUNCTION {format.date}
{ year empty$
    { month empty$
 { "" }
 { "there's a month but no year in " cite$ * warning$
   month
 }
      if$
    }
    { month empty$
 'year
 { month " " * year * }
      if$
    }
  if$
}

FUNCTION {format.btitle}
{ title emphasize
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}

FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { "volume" volume tie.or.space.connect
      series empty$
 'skip$
 { " of " * series emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION {format.number.series}
{ volume empty$
    { number empty$
 { series field.or.null }
 { output.state mid.sentence =
     { "number" }
     { "Number" }
   if$
   number tie.or.space.connect
   series empty$
     { "there's a number but no series in " cite$ * warning$ }
     { " in " * series * }
   if$
 }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { output.state mid.sentence =
 { edition "l" change.case$ " edition" * }
 { edition "t" change.case$ " edition" * }
      if$
    }
  if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
 { #1 'multiresult := }
 { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { pages multi.page.check
 { "pages" pages n.dashify tie.or.space.connect }
 { "page" pages tie.or.space.connect }
      if$
    }
  if$
}

FUNCTION {format.vol.num.pages}
{ volume field.or.null
  number empty$
    'skip$
    { "(" number * ")" * *
      volume empty$
 { "there's a number but no volume in " cite$ * warning$ }
 'skip$
      if$
    }
  if$
  pages empty$
    'skip$
    { duplicate$ empty$
 { pop$ format.pages }
 { ":" * pages n.dashify * }
      if$
    }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
 { "chapter" }
 { type "l" change.case$ }
      if$
      chapter tie.or.space.connect
      pages empty$
 'skip$
 { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
    { "" }
    { editor empty$
 { "In " booktitle emphasize * }
 { "In " format.editors * ", " * booktitle emphasize * }
      if$
    }
  if$
}

FUNCTION {empty.misc.check}

{ author empty$ title empty$ howpublished empty$
  month empty$ year empty$ note empty$
  and and and and and
  key empty$ not and
    { "all relevant fields are empty in " cite$ * warning$ }
    'skip$
  if$
}

FUNCTION {format.thesis.type}
{ type empty$
    'skip$
    { pop$
      type "t" change.case$
    }
  if$
}

FUNCTION {format.tr.number}
{ type empty$
    { "Technical Report" }
    'type
  if$
  number empty$
    { "t" change.case$ }
    { number tie.or.space.connect }
  if$
}

FUNCTION {format.article.crossref}
{ key empty$
    { journal empty$
 { "need key or journal for " cite$ * " to crossref " * crossref *
   warning$
   ""
 }
 { "In {\em " journal * "\/}" * }
      if$
    }
    { "In " key * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
  editor num.names$ duplicate$
  #2 >
    { pop$ " et~al." * }
    { #2 <
 'skip$
 { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
     { " et~al." * }
     { " and " * editor #2 "{vv~}{ll}" format.name$ * }
   if$
 }
      if$
    }
  if$
}

FUNCTION {format.book.crossref}
{ volume empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      "In "
    }
    { "Volume" volume tie.or.space.connect
      " of " *
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { series empty$
     { "need editor, key, or series for " cite$ * " to crossref " *
       crossref * warning$
       "" *
     }
     { "{\em " * series * "\/}" * }
   if$
 }
 { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { booktitle empty$
     { "need editor, key, or booktitle for " cite$ * " to crossref " *
       crossref * warning$
       ""
     }
     { "In {\em " booktitle * "\/}" * }
   if$
 }
 { "In " key * }
      if$
    }
    { "In " format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { journal emphasize "journal" output.check
      format.vol.num.pages output
      format.date "year" output.check
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull
      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  format.authors output
  new.block
  format.title "title" output.check
  howpublished address new.block.checkb
  howpublished output
  address output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull

      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.chapter.pages output
      new.sentence
      publisher "publisher" output.check
      address output
      format.edition output
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.pages output
      address empty$
 { organization publisher new.sentence.checkb
   organization output
   publisher output
   format.date "year" output.check
 }
 { address output.nonnull
   format.date "year" output.check
   new.sentence
   organization output
   publisher output
 }
      if$
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization empty$
 'skip$
 { organization output.nonnull
   address output
 }
      if$
    }
    { format.authors output.nonnull }
  if$
  new.block
  format.btitle "title" output.check
  author empty$
    { organization empty$
 { address new.block.checka
   address output
 }
 'skip$
      if$
    }
    { organization address new.block.checkb
      organization output
      address output
    }
  if$
  format.edition output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  "Master's thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  title howpublished new.block.checkb
  format.title output
  howpublished new.block.checka
  howpublished output
  format.date output
  new.block
  note output
  fin.entry
  empty.misc.check
}

FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.btitle "title" output.check
  new.block
  "PhD thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization output }
    { format.editors output.nonnull }

  if$
  new.block
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  address empty$
    { editor empty$
 { publisher new.sentence.checka }
 { organization publisher new.sentence.checkb
   organization output
 }
      if$
      publisher output
      format.date "year" output.check
    }
    { address output.nonnull
      format.date "year" output.check
      new.sentence
      editor empty$
 'skip$
 { organization output }
      if$
      publisher output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  note "note" output.check
  format.date output
  fin.entry
}

FUNCTION {default.type} { misc }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sept."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Softw. Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput.-Aided Design Integrated Circuits"}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Programming"}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Gr."}

MACRO {toms} {"ACM Trans. Math. Softw."}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Prog. Lang. Syst."}

MACRO {tcs} {"Theoretical Comput. Sci."}

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
 { "   " * }
 'skip$
      if$
      s nameptr "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
 { "et al" * }
 { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
 { "to sort, need author or key in " cite$ * warning$
   ""
 }
 { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
 { key empty$
     { "to sort, need author, editor, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.organization.sort}
{ author empty$

    { organization empty$
 { key empty$
     { "to sort, need author, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.organization.sort}
{ editor empty$
    { organization empty$
 { key empty$
     { "to sort, need editor, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {presort}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
 'editor.organization.sort
 { type$ "manual" =
     'author.organization.sort
     'author.sort
   if$
 }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { longest.label }

INTEGERS { number.label longest.label.width }

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #1 'number.label :=
  #0 'longest.label.width :=
}

FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
  number.label #1 + 'number.label :=
  label width$ longest.label.width >
    { label 'longest.label :=
      label width$ 'longest.label.width :=
    }
    'skip$
  if$
}

EXECUTE {initialize.longest.label}

ITERATE {longest.label.pass}

FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{"  longest.label  * "}" *
  "\itemsep=-1pt" * % Compact the entries a little.
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}

% end of file ieee.bst
% ---------------------------------------------------------------




